Visual Pivoting for (Unsupervised) Entity Alignment

This work studies the use of visual semantic representations to align entities in heterogeneous knowledge graphs (KGs). Images are natural components of many existing KGs. By combining visual knowledge with other auxiliary information, we show that the proposed new approach, EVA, creates a holistic entity representation that provides strong signals for cross-graph entity alignment. Besides, previous entity alignment methods require human labelled seed alignment, restricting availability. EVA provides a completely unsupervised solution by leveraging the visual similarity of entities to create an initial seed dictionary (visual pivots). Experiments on benchmark data sets DBP15k and DWY15k show that EVA offers state-of-the-art performance on both monolingual and cross-lingual entity alignment tasks. Furthermore, we discover that images are particularly useful to align long-tail KG entities, which inherently lack the structural contexts necessary for capturing the correspondences.

==> includes/backups.tex <==

\begin{table*}[!htbp]
\scriptsize
%\setlength{\tabcolsep}{0.1em}
\setlength{\tabcolsep}{0.8pt}
%\vspace*{-0.3cm}
%\renewcommand{\arraystretch}{0.8}
\caption{Quantitative results on DBP15k. Comparison with related works with and without using iterative learning.}
\label{Table:5}
\centering
\begin{tabular}{cclccccccccccccccccccccccccccccc}
\toprule
 \multirow{2}{*}{\#} & & \multirow{2}{*}{model} &     &  \multicolumn{4}{c}{FR$\rightarrow$EN} & & \multicolumn{4}{c}{FR$\leftarrow$EN} &   \multicolumn{4}{c}{JA$\rightarrow$EN} & & \multicolumn{4}{c}{JA$\leftarrow$EN} & \multicolumn{4}{c}{ZH$\rightarrow$EN} & & \multicolumn{4}{c}{ZH$\leftarrow$EN} \\
 \cmidrule{4-7}\cmidrule{9-12}\cmidrule{14-17} \cmidrule{19-22} \cmidrule{24-27} \cmidrule{29-32}
 & & &  H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR \\
\midrule 
 & \multirow{4}{*}{\rotatebox[origin=c]{90}{w/o iter.}} & \citep{li2019semi} & .486 & .851 & - & .610 & & - & - & - & -  & & .490  & .844 & - &.610 & & - & - & - & - & &.478 & .835 & - & .598 & & - & - & - & - \\
 \\
 \\
 & & our model & .731 & .937 & .978 & .805 & & .732 & .937  & .978 & .806 & & .716 & .926 & .971 & .791 & & .724 & .926 & .971 & .796 & &.715 & .923 & .970 & .791 & & .713 & .923  & .969 & .789  \\
\midrule
& \multirow{5}{*}{\rotatebox[origin=c]{90}{w/ iter.}} &  \\
& & \\
& & \\
& & our model & .770 & .954 & .984 & .837 & & .771 & .955 & .984 & .838 & & .761 & .945 & .978 & .829 & & .766 & .936 & .974 & .828 & & .771 & .932 & .972 & .830 & & .768 & .932 & .972 & .828  \\
\bottomrule
\end{tabular}
%\vspace{-0.1cm}
\end{table*}


\begin{table*}[!htbp]
\scriptsize
%\setlength{\tabcolsep}{0.1em}
\setlength{\tabcolsep}{0.8pt}
%\vspace*{-0.3cm}
%\renewcommand{\arraystretch}{0.8}
\caption{Quantitative results on DBP15k. Ablation studies on side information used. Without iterative learning.}
\label{Table:5}
\centering
\begin{tabular}{clccccccccccccccccccccccccccccc}
\toprule
 \multirow{2}{*}{\#} & \multirow{2}{*}{model} &     &  \multicolumn{4}{c}{FR$\rightarrow$EN} & & \multicolumn{4}{c}{FR$\leftarrow$EN} &   \multicolumn{4}{c}{JA$\rightarrow$EN} & & \multicolumn{4}{c}{JA$\leftarrow$EN} & \multicolumn{4}{c}{ZH$\rightarrow$EN} & & \multicolumn{4}{c}{ZH$\leftarrow$EN} \\
 \cmidrule{4-6}\cmidrule{8-11}\cmidrule{13-16} \cmidrule{18-21} \cmidrule{23-26} \cmidrule{28-31}
 & &   H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR \\
\midrule 
& full model w/o structure & .403 & .584 & .766 & .463 & & .408 & .584 & .775 & .465 & & .416 & .610 & .786 & .481 & & .413 & .623 & .792 & .483 & & .429 & .649 & .821 & .502 & & .430 & .639 & .814 & .499 \\
& full model w/o attribute & .688 & .914 & .964 & .768 & & .691 & .914 & .964 & .770 & & \\
& full model w/o relation & .696 & .924 & .971 &.778 & & .700 & .922 & .970 & .780 \\
& full model w/o image & .668 & .920 & .969 & .759 & & .675 & .918 & 970 & .762 & & .656 & .901 & .960 & .746 & & .659 & .903 & .959 & .747 & & .657 & .905 & .959 & .746  & & .657 & .903 & .959 & .747\\
& full model  & .731 & .937 & .978 & .805 & & .732 & .937  & .978 & .806 & & .716 & .926 & .971 & .791 & & .724 & .926 & .971 & .796 & &.715 & .923 & .970 & .791 & & .713 & .923  & .969 & .789 \\
\bottomrule
\end{tabular}
%\vspace{-0.1cm}
\end{table*}



\begin{table*}[!htbp]
\scriptsize
\setlength{\tabcolsep}{0.8pt}
%\vspace*{-0.3cm}
%\renewcommand{\arraystretch}{0.8}
\caption{Quantitative results on DBP15k. Unsupervised setting.}
\label{Table:5}
\centering
\begin{tabular}{cclccccccccccccccccccccccccccccc}
\toprule
 \multirow{2}{*}{\#} &\multirow{2}{*}{seed} & \multirow{2}{*}{model}   &  \multicolumn{4}{c}{FR$\rightarrow$EN} & & \multicolumn{4}{c}{FR$\leftarrow$EN} & & \multicolumn{4}{c}{JA$\rightarrow$EN} & & \multicolumn{4}{c}{JA$\leftarrow$EN} & &  \multicolumn{4}{c}{ZH$\rightarrow$EN} & & \multicolumn{4}{c}{ZH$\leftarrow$EN}  \\
 \cmidrule{4-7}\cmidrule{9-12} \cmidrule{14-17}\cmidrule{19-22}\cmidrule{24-27} \cmidrule{29-32}
  & & &  H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR & & H1 & H10 & H50 & MRR\\
  \midrule
& 100 & full model (std)  & .578 & .822 & .919 & .661 & & .581 & .821 & .918 & .664 & &  .550 & .764 & .868 & .624 & & .547 & .767 & .8651 & .623 & & .573 & .783 & .877 & .645 & & .577 & .780 & .877 & .647  \\
& 300 & full model (std) & \\ %.488 & .755 & .884 & .580 & & .487 & .754 & .881 & .580 & & .415 & .674 & .816 & .503 & &  .417 &.673  & .812 &.505 \\
& 500 & full model (std) &  \\ %.579 & .825 & .919 & .665 & & .578 & .825 & .920 & .665 & & .489 & .757 & .877 & .581 & & .490 & .756 &.876 & .582 & & .573 & .809 & .904 & .655 & & .576 & .808 & .902 & .658 \\
& 1000 & full model (std) & \\ %.634 & .863 & .945 & .715 & & .636 & .865 & .943 & .716 & & .579 & .826 & .920 & .664 & & .579 & .820 & .918 & .665 \\
& 2000 & full model (std)  &  \\ %.675 & .880 & .952 & .746 & & .677 & .879 & .953 & .748 & & .647 & .854 & 0.928 & .721 & & .645 & .855 & .931 & .719 \\
& 3000 & full model (std)  & .681 & .883 & .955 & .748 & & .678 & .884 & .953 & .747  \\ %.726 & .912 & .972 & .794 & & .726 & .919 & .975 & .794 & & .699 & .896 & .961 & .769 & & .697 & .898 & .959 & .768 \\
& 4000 & full model (std)  &  .699 & .893 & .959 & .765  & & .700 & .895 & .961 & .766 \\ % .726 & .914 & .969 & .793 & & .729 & .915 & .970 & .795 & & .727 & .910 & .966 & .791 & & .723 & .911 & .966 & .790 \\
& 5000 & full model (std)  & .690 & .889 & .954 & .758 & & .697 & .891 & .954  & .762 & & .690 & .879 & .946 & .756 & & .695 & .881 & .946 & .760 & & .711 & .876 & .935 & .769 && .710  &.876 & .936 & .768  \\  %.732 & .919 & .975 & .798 & & .731 & .929 & .975 & .798 & & .727 & .905 & .964 & .790 & & .727 & .910 & .963 & .792 \\
\midrule
& supervised & full model (std)  & .763 & .947 & .982 & .831 & & .762 & .949 & .981 & .831 & & .761 & .945 & .978 & .829 & & .761 & .944 & .977 & .829  & & .764 & .941 & .980 &.829 & & .765 &.942 & .981 & .830  \\
\bottomrule
\end{tabular}
%\vspace{-0.1cm}
\end{table*}


==> includes/discuss.tex <==
\section{Discussion}
